Domain Guidance: A Simple Transfer Approach for a Pre-trained Diffusion Model

Recent advancements in diffusion models have revolutionized generative modeling. However, the impressive and vivid outputs they produce often come at the cost of significant model scaling and increased computational demands. Consequently, building personalized diffusion models based on off-the-shelf models has emerged as an appealing alternative. In this paper, we introduce a novel perspective on conditional generation for transferring a pre-trained model. From this viewpoint, we propose *Domain Guidance*, a straightforward transfer approach that leverages pre-trained knowledge to guide the sampling process toward the target domain. Domain Guidance shares a formulation similar to advanced classifier-free guidance, facilitating better domain alignment and higher-quality generations. We provide both empirical and theoretical analyses of the mechanisms behind Domain Guidance. Our experimental results demonstrate its substantial effectiveness across various transfer benchmarks, achieving over a 19.6% improvement in FID and a 23.4% improvement in FD$_\text{DINOv2}$ compared to standard fine-tuning. Notably, existing fine-tuned models can seamlessly integrate Domain Guidance to leverage these benefits, without additional training.

==> tabs/tab_big_full_table.tex <==
\begin{table*}[t]
    \setlength{\abovecaptionskip}{-0.01cm}
    \setlength{\belowcaptionskip}{-0.1cm}
    \caption{Quantitative results on downstream tasks with pre-trained DiT-XL-2-256x256.}
    \vskip 0.1in
    \centering
    \setlength{\tabcolsep}{2.0pt}
    \scalebox{0.9}{
    \begin{tabular}{c|c|ccccccc|c}
    \toprule
    Metrics & \makecell[c]{~Method~}&\makecell[c]{~Food~} & ~SUN~ & \makecell[c]{DF-20M}  & \makecell[c]{Caltech}  & \makecell[c]{CUB-Bird} & \makecell[c]{ArtBench}  & \makecell[c]{ Cars} &  \makecell[c]{Average} \\
    \midrule
    \multirow{3}{*}{FID $\downarrow$} & Standard Fine-tuning                & 16.04 & \underline{14.74} & 29.79 & 5.32 & 20.59 & 16.67 & 6.04 & 14.36
    \\
    & + Classifier-free Guidance          & 10.68 & 11.01 & \underline{14.74}  & 5.32 & 20.59 & 16.67 & 6.04 & 14.36\\
    % \midrule
    & + \textbf{Domain Guidance}          & \textbf{16.04}  & \textbf{12.57} & \textbf{23.79} & \textbf{3.50} & \textbf{13.85} & \textbf{12.64} & \textbf{5.37} & \textbf{10.63} \\
    \midrule
    \multirow{3}{*}{FD$_\text{DINOv2}$ $\downarrow$} & Standard Fine-tuning                & 16.04 & \underline{14.74} & 29.79 & 5.32 & 20.59 & 16.67 & 6.04 & 14.36
    \\
    & + Classifier-free Guidance          & 10.68 & 11.01 & \underline{14.74}  & 5.32 & 20.59 & 16.67 & 6.04 & 14.36\\
    % \midrule
    & + \textbf{Domain Guidance}          & \textbf{16.04}  & \textbf{12.57} & \textbf{23.79} & \textbf{3.50} & \textbf{13.85} & \textbf{12.64} & \textbf{5.37} & \textbf{10.63} \\
    \midrule
    \multirow{3}{*}{Precision $\uparrow$} & Standard Fine-tuning                & 16.04 & \underline{14.74} & 29.79 & 5.32 & 20.59 & 16.67 & 6.04 & 14.36
    \\
    & + Classifier-free Guidance          & 10.68 & 11.01 & \underline{14.74}  & 5.32 & 20.59 & 16.67 & 6.04 & 14.36\\
    % \midrule
    & + \textbf{Domain Guidance}          & \textbf{16.04}  & \textbf{12.57} & \textbf{23.79} & \textbf{3.50} & \textbf{13.85} & \textbf{12.64} & \textbf{5.37} & \textbf{10.63} \\
    % Relative Promotion & 43.4\% & 34.5\% & 14.7\% & 20.1\% & 34.2\% & 32.7\% & 24.2\% & 11.1\% & 26.0\% \\
    \midrule
    \multirow{3}{*}{Recall $\uparrow$} & Standard Fine-tuning                & 16.04 & \underline{14.74} & 29.79 & 5.32 & 20.59 & 16.67 & 6.04 & 14.36
    \\
    & + Classifier-free Guidance          & 10.68 & 11.01 & \underline{14.74}  & 5.32 & 20.59 & 16.67 & 6.04 & 14.36\\
    % \midrule
    & + \textbf{Domain Guidance}          & \textbf{16.04}  & \textbf{12.57} & \textbf{23.79} & \textbf{3.50} & \textbf{13.85} & \textbf{12.64} & \textbf{5.37} & \textbf{10.63} \\
    % Relative Promotion & 43.4\% & 34.5\% & 14.7\% & 20.1\% & 34.2\% & 32.7\% & 24.2\% & 11.1\% & 26.0\% \\
    \bottomrule 
    \end{tabular}
    }
    \vspace{0.5cm}
    \label{table: fine-tuning-downstream-datasets-big}
    \vspace{-0.3cm}
\end{table*}
